Density-dependent effective baryon-baryon interaction from chiral three-baryon forces

A density-dependent effective potential for the baryon-baryon interaction in the presence of the (hyper)nuclear medium is constructed, based on the leading (irreducible) three-baryon forces derived within SU(3) chiral effective field theory. We evaluate the contributions from three classes: contact terms, one-pion exchange and two-pion exchange. In the strangeness-zero sector we recover the known result for the in-medium nucleon-nucleon interaction. Explicit expressions for the Lambda-nucleon in-medium potential in (asymmetric) nuclear matter are presented. Our results are suitable for implementation into calculations of (hyper)nuclear matter. In order to estimate the low-energy constants of the leading three-baryon forces we introduce the decuplet baryons as explicit degrees of freedom and construct the relevant terms in the minimal non-relativistic Lagrangian. With these, the constants are estimated through decuplet saturation. Utilizing this approximation we provide numerical results for the effect of the three-body force in symmetric nuclear matter and pure neutron matter on the Lambda-nucleon interaction. A moderate repulsion that increases with density is found in comparison to the free Lambda-nucleon interaction.

==> files/DBBBSm1.tex <==
-1 & \Lambda N \to \Delta \Sigma & \frac{1}{2} & \frac{\lC_1 +3 \lC_2 }{\sqrt{3}} \\ 
-1 & \Lambda N \to \Sigma^*  N & \frac{1}{2} & \frac{\lC_1 +3 \lC_2 }{2 \sqrt{3}} \\ 
-1 & \Sigma N \to \Delta \Sigma & \frac{1}{2} & -\frac{\lC_1 +3 \lC_2 }{\sqrt{3}} \\ 
-1 & \Sigma N \to \Delta \Sigma & \frac{3}{2} & \sqrt{\frac{5}{6}} \lC_1  \\ 
-1 & \Sigma N \to \Delta \Lambda & \frac{3}{2} & \frac{\lC_1 }{\sqrt{6}} \\ 
-1 & \Sigma N \to \Sigma^*  N & \frac{1}{2} & -\frac{\lC_1 +3 \lC_2 }{2 \sqrt{3}} \\ 
-1 & \Sigma N \to \Sigma^*  N & \frac{3}{2} & \frac{\lC_1 }{\sqrt{3}} \\ 


==> files/DBBBSm2.tex <==
-2 & \Xi N \to \Delta \Xi & 1 & -\frac{2 \lC_2 }{\sqrt{3}} \\ 
-2 & \Xi N \to \Sigma^*  \Sigma & 0 & \frac{\lC_1 +3 \lC_2 }{\sqrt{2}} \\ 
-2 & \Xi N \to \Sigma^*  \Sigma & 1 & -\frac{\lC_1 +\lC_2 }{\sqrt{3}} \\ 
-2 & \Xi N \to \Sigma^*  \Lambda & 1 & -\frac{\lC_1 +3 \lC_2 }{3 \sqrt{2}} \\ 
-2 & \Xi N \to \Xi^*  N & 0 & \frac{\lC_1 +3 \lC_2 }{\sqrt{3}} \\ 
-2 & \Xi N \to \Xi^*  N & 1 & -\frac{\lC_1 +\lC_2 }{\sqrt{3}} \\ 
-2 & \Sigma \Lambda \to \Delta \Xi & 1 & \frac{\sqrt{2} \lC_1 }{3} \\ 
-2 & \Sigma \Lambda \to \Sigma^*  \Sigma & 1 & -\frac{\sqrt{2} \lC_1 }{3} \\ 
% -2 & \Sigma \Lambda \to \Xi^*  N & 1 & -\frac{\sqrt{2} \lC_1 }{3} \\ 
% -2 & \Sigma \Sigma \to \Delta \Xi & 1 & \frac{2 (\lC_1 +2 \lC_2 )}{\sqrt{3}} \\ 
% -2 & \Sigma \Sigma \to \Sigma^*  \Sigma & 1 & \frac{2 \lC_2 }{\sqrt{3}} \\ 
% -2 & \Sigma \Sigma \to \Sigma^*  \Lambda & 1 & \frac{1}{3} \sqrt{2} (\lC_1 +3 \lC_2 ) \\ 
% -2 & \Sigma \Sigma \to \Xi^*  N & 1 & \frac{2 \lC_2 }{\sqrt{3}} \\ 


==> files/DBBBSm3.tex <==
-2 & \Sigma \Lambda \to \Xi^*  N & 1 & -\frac{\sqrt{2} \lC_1 }{3} \\ 
-2 & \Sigma \Sigma \to \Delta \Xi & 1 & \frac{2 (\lC_1 +2 \lC_2 )}{\sqrt{3}} \\ 
-2 & \Sigma \Sigma \to \Sigma^*  \Sigma & 1 & \frac{2 \lC_2 }{\sqrt{3}} \\ 
-2 & \Sigma \Sigma \to \Sigma^*  \Lambda & 1 & \frac{1}{3} \sqrt{2} (\lC_1 +3 \lC_2 ) \\ 
-2 & \Sigma \Sigma \to \Xi^*  N & 1 & \frac{2 \lC_2 }{\sqrt{3}} \\ \cmidrule(l){1-3}\cmidrule(lr){4-4}
%
-3 & \Xi \Lambda \to \Sigma^*  \Xi & \frac{1}{2} & -\frac{\lC_1 -3 \lC_2 }{2 \sqrt{3}} \\ 
-3 & \Xi \Lambda \to \Xi^*  \Sigma & \frac{1}{2} & \frac{2 \lC_1 +3 \lC_2 }{2 \sqrt{3}} \\ 
-3 & \Xi \Lambda \to \Xi^*  \Lambda & \frac{1}{2} & \frac{\sqrt{3} \lC_2 }{2} \\ 
-3 & \Xi \Lambda \to \Omega N & \frac{1}{2} & \frac{2 \lC_1 +3 \lC_2 }{\sqrt{6}} \\ 
-3 & \Xi \Sigma \to \Sigma^*  \Xi & \frac{1}{2} & -\frac{1}{2} \sqrt{3} (\lC_1 +\lC_2 ) \\ 
-3 & \Xi \Sigma \to \Xi^*  \Sigma & \frac{1}{2} & -\frac{\sqrt{3} \lC_2 }{2} \\ 
-3 & \Xi \Sigma \to \Xi^*  \Lambda & \frac{1}{2} & -\frac{2 \lC_1 +3 \lC_2 }{2 \sqrt{3}} \\ 
-3 & \Xi \Sigma \to \Omega N & \frac{1}{2} & -\sqrt{\frac{3}{2}} \lC_2  \\ 


==> files/DBBBSm4.tex <==
-4 & \Xi \Xi \to \Xi^*  \Xi & 0 & \frac{2 \lC_1 }{\sqrt{3}} \\ 
-4 & \Xi \Xi \to \Omega \Lambda & 0 & \frac{2 \lC_1 }{\sqrt{3}} \\ 

